ConceptLens: from Pixels to Understanding

ConceptLens is an innovative tool designed to illuminate the intricate workings of deep neural networks (DNNs) by visualizing hidden neuron activations. By integrating deep learning with symbolic methods, ConceptLens offers users a unique way to understand what triggers neuron activations and how they respond to various stimuli. The tool uses error-margin analysis to provide insights into the confidence levels of neuron activations, thereby enhancing the interpretability of DNNs. This paper presents an overview of ConceptLens, its implementation, and its application in real-time visualization of neuron activations and error margins through bar charts.

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}


% ------- Discussion Points ----- 
% 1. 
The error margins derived from our analysis significantly enhance the interpretability and reliability of neural networks. These margins provide a quantitative measure of confidence for concept detection in image analysis tasks. For instance, when a neuron associated with a specific concept (e.g., "buffet") activates above a certain threshold, the error margin allows us to estimate the likelihood that the image actually contains that concept. 

Our study demonstrates the robustness of error margin methodology across diverse datasets without assuming identical neuron-concept associations between Google Images and ADE20K. Instead, our primary goal was to validate the generalizability of error margins across these distinct datasets. In our experiments, we observed varying neuron-concept associations across datasets. For instance, while neuron 62 prominently associated with 'buffet' in Google Images, its activation pattern in ADE20K showed similarities but also notable differences. These variations stem from differences in dataset characteristics, training specificity, and concept granularity. Importantly, these differences strengthen our findings. The methodology's ability to produce statistically significant results despite these variations underscores its robustness and broad applicability. This adaptability is crucial for real-world applications requiring reliable concept detection and interpretability across diverse data contexts.

Our statistical analysis, employing Mann-Whitney U and Wilcoxon signed-rank tests, reveals significant differences in non-target label activations (Non-TLA) between the ADE20K dataset and the Google Images dataset. Crucially, the lower Non-TLA values observed in the ADE20K dataset validate our error margins and underscore their reliability. This validation is important for several reasons:

\begin{itemize}
    \item \textbf{Generalizability}: The fact that error margins derived from the Google Images dataset generalize well to the more structured and annotated ADE20K dataset indicates that our method is not confined to a specific dataset. This enhances the broader applicability of our approach.
    \item \textbf{Reliability}: The reduced Non-TLA in the ADE20K dataset suggests that neuron activation patterns are more precise and reliable when tested on a well-annotated dataset. This finding assures that the calculated error margins are robust and can be trusted for practical AI applications.
    \item \textbf{Foundation for Future Work}: Validating our error margins across different datasets provides a strong foundation for future research, encouraging further exploration of neuron activation patterns and their implications for model explainability.
\end{itemize}

These error margins significantly enhance the interpretability of neural network decisions by quantifying the reliability of neuron-concept associations. This offers a more nuanced understanding of how the network processes information, going beyond simple neuron labeling to provide insights into the degree of certainty with which we can interpret a neuron's activation. Such information is crucial for building trust in AI systems, especially in critical decision-making scenarios.

Furthermore, our error margin analysis can guide the refinement of neural architectures. By identifying neurons or neuron ensembles with high precision for specific concepts, we can inform targeted improvements in network design. For example, architectures could be optimized to enhance the precision of key concept detections, potentially leading to more efficient and accurate models.

In summary, our analysis demonstrates that the concept associations and error margins derived from our method are both reliable and generalizable. These findings contribute significantly to the field of explainable AI by providing a validated approach to understanding and improving the interpretability of neural networks, paving the way for more advanced and trustworthy AI systems.

==> sections/literature.tex <==
\subsection{Related work}
\label{sec:literature_review}


Efforts to demystify deep learning~\cite{gunning2019xai,adadi2018peeking,minh2022explainable} are ongoing. Methods for explainability can be categorized based on their approach to understanding input data, such as feature summarization~\cite{selvaraju2016grad,lime_rebeiro}, or the model's internal representation, like node summarization~\cite{zhou2018interpreting,bau2020understanding}. These methods further classify into model-specific~\cite{selvaraju2016grad} or model-agnostic~\cite{lime_rebeiro} approaches. Some methods rely on human interpretation of explanatory data, such as posing counterfactual questions~\cite{DBLP:journals/corr/abs-1711-00399}.


Model-agnostic techniques for feature attribution, such as LIME~\cite{lime_rebeiro} and SHAP~\cite{shap_lundberg}, aim to elucidate model predictions by assessing the influence of individual features. However, they encounter challenges like explanation instability~\cite{attacklime_alvarez} and susceptibility to biased classifiers~\cite{attacklimeandshap_lakkaraju}. On the other hand, pixel attribution endeavors to comprehend predictions by assigning significance to individual pixels~\cite{saliencymap_simonyan,gradcam_batra,smoothgrad_smilkov}. Nonetheless, it faces notable limitations, particularly with ReLU activation~\cite{gradcamattack_shrikumar} and adversarial perturbations~\cite{unreliablepixelattribution_kim}, leading to inconsistencies in interpretability.

Explanations developed by \cite{tcav_kim,tcar_crabbe} employ supervised learning and curated concepts. These methods utilize classifiers on target concepts, with weights representing Concept Activation Vectors (CAVs). Another approach by \cite{ace_ghorbani} utilizes image segmentation and clustering for concept selection, albeit potentially losing information and only applicable to visible concepts. \cite{invertibletcav_zhang} proposed enhancements using Non-negative Matrix Factorization to mitigate information loss. Individual Conditional Expectation (ICE) plots~\cite{ice_goldstein} and Partial Dependency Plots~\cite{pdp_friedman} provide insights into prediction-feature relationships from both local and global perspectives but may struggle with intricate feature interactions.

 
Previous studies suggest that hidden neurons may represent high-level concepts~\cite{zhou2018interpreting,bau2020understanding}, but these methods often require semantic segmentation~\cite{xiao2018unified} (resource-intensive) or explicit concept annotations~\cite{tcav_kim}. 

Some research have utilized Semantic Web data for explaining deep learning models~\cite{confalonieri2021using,diaz2022explainable}, and Concept Induction for providing explanations~\cite{sarker2017explaining,9736291}. However, their focus was on analyzing input-output behavior, generating explanations for the overall system. 
% In contrast, we concentrate on understanding internal node activations.

CLIP-Dissect~\cite{oikarinen2022clip} represents work similar to ours, employing a different approach. They utilize the CLIP pre-trained model, employing zero-shot learning to associate images with labels. Label-Free Concept Bottleneck Models~\cite{oikarinen2023label}, building upon CLIP-Dissect, use GPT-4~\cite{achiam2023gpt} for concept set generation.
However, CLIP-Dissect has limitations that may be challenging to overcome without significant changes to the approach. These include limited accuracy in predicting output labels based on concepts in the last hidden layer and difficulty in transferring to other modalities or domain-specific applications. The Label-Free approach inherits these limitations and may compromise explainability, as it uses a concept derivation method that is not inherently explainable.



==> sections/preliminaries.tex <==
\section{Preliminaries}



==> sections/results.tex <==
\section{Results}
\label{sec:results}



Our findings suggest that our methodology for assigning \textit{error-margins} for image predictions is not only reliable but also generalizable across diverse datasets, confirmed by statistical evaluation. 

Table~\ref{tab:stats_eval} demonstrates a consistent trend of decreased Non-TLA\% in the ADE20k dataset compared to Google Images across various threshold categories. Among the 33 hypotheses tested for the category of non-target activations $>$ 0, 13 were rejected at a significance level of p $<$ 0.05. Similarly, for the category of non-target activations $>$ 20\%, 15 hypotheses were rejected at the same significance level. In the case of non-target activations $>$ 40\%, 21 hypotheses were rejected, while for non-target activations $>$ 60\%, 23 hypotheses were rejected, all at a p-value $<$ 0.05. These findings underscore a consistent and statistically significant decrease in non-target activations in the ADE20k dataset, indicating its potential for robust image analysis tasks.

The Wilcoxon signed rank test results further reinforce this trend. Across various thresholds, the test consistently indicated a decrease in non-target activations in the ADE20k dataset compared to Google Images. This trend was particularly evident when considering all threshold categories together, where the p-value was found to be $<$ 0.05, leading to the rejection of the null hypothesis. This suggests that the error estimates obtained from the Google image data are reliable and are either maintained or even surpassed by the ADE20k images, highlighting the potential of leveraging ADE20k for image analysis tasks, particularly in scenarios where minimizing error rates is crucial. This comparative analysis offers valuable insights for refining image analysis methodologies and informs future research directions in this domain.



